LLaMA-Berry: Pairwise Optimization for O1-like Olympiad-Level Mathematical Reasoning

This paper presents an advanced mathematical problem-solving framework, LLaMA-Berry, for enhancing the mathematical reasoning ability of Large Language Models (LLMs). The framework combines Monte Carlo Tree Search (MCTS) with iterative Self-Refine to optimize the reasoning path and utilizes a pairwise reward model to evaluate different paths globally. By leveraging the self-critic and rewriting capabilities of LLMs, Self-Refine applied to MCTS (SR-MCTS) overcomes the inefficiencies and limitations of conventional step-wise and greedy search algorithms by fostering a more efficient exploration of solution spaces. Pairwise Preference Reward Model~(PPRM), inspired by Reinforcement Learning from Human Feedback (RLHF), is then used to model pairwise preferences between solutions, utilizing an Enhanced Borda Count (EBC) method to synthesize these preferences into a global ranking score to find better answers. This approach addresses the challenges of scoring variability and non-independent distributions in mathematical reasoning tasks. The framework has been tested on general and advanced benchmarks, showing superior performance in terms of search efficiency and problem-solving capability compared to existing methods like ToT and rStar, particularly in complex Olympiad-level benchmarks, including GPQA, AIME24 and AMC23.

==> backup/baseline_with_base_methods.tex <==
% \cn{这个表的目的是固定住base model，和tree of thoughts,self consistency CoT,Self-refine,CoT方法进行比较}

\begin{table}[!htbp]
\centering
\caption{Performance of Different Tree-based Methods Based on LLaMA 3-8B}
\label{tab:different-trees-benchmark}
\scriptsize
\setlength{\tabcolsep}{3pt} % Adjust column separation
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c|c}
\hline
\multicolumn{1}{c|}{\diagbox{Method}{Benchmark}} & GSM8K & GSM-HARD & MATH500 \\
\hline
Zero-Shot CoT                  & 68.4  & 14.9  & 5.8  \\ 
Few-shot CoT                   & 74.5  & 25.6  & 17.8 \\ 
One-turn Self-Refine           & 75.7  & 26.5  & 25.0 \\ 
Self-Consistency with 8 Samplings & 78.4@major8 & 28.5@major8 & 30.0@major8 \\ 
Self-Consistency with 64 Samplings & 83.2@major64 & 30.3@major64 & 33.0@major64 \\ 
Self-Consistency with 128 Samplings & 84.7@major128 & 31.2@major128 & 33.8@major128 \\ 
Tree of Thoughts               & 69.1  & 19.6  & 13.6 \\ 
Reasoning via Planning          & 80.6  & 29.6  & 18.8 \\
rStar with 32 Rollouts          & 88.7@major32 & 33.4@major32 & 38.3@major32 \\ 
rStar with mutual reasoning, 32 Rollouts & 91.7 & 37.5 & 42.9 \\  \hline
\multirow{2}{*}{\textbf{MCTSr with 8 Rollouts}} & 86.4@major8 & 30.2@major8 & 35.2@major8 \\
                                                & 94.1@rm8  & 37.1@rm8  & 56.4@rm8  \\  \hline
\multirow{2}{*}{\textbf{MCTSr with 16 Rollouts}} & 88.1@major16 & 31.5@major16 & 39.6@major16 \\
                                                & 96.4@rm16 & 41.1@rm16 & 63.8@rm16 \\
\hline
\end{tabular}}
\end{table}



==> backup/methods.tex <==


% 这里讲的太快了。建议改为，我们要解决的大科学问题简介，里面的核心问题是什么(例如求解value function，或者policy function)，最后一两句话点题，本文就是为了解决这个核心问题。

% For solutions of mathematical problem-solving tasks, a reasoning path could be generated in step-wise or path-wise. The action space of step-wise is nearly infinite which makes reasoning hard to control and improve. We formalize this task as a path-wise Markov Decision Process~(MDP) framework, the state space, denoted as \( S \), encapsulates each state \( s \) as a complete problem-solving answer. Actions within this context, represented by the action space \( A \), comprise all possible rewriting operations that transition a current state \( s \) to a new state \( s' \) through the state transition function \( T \), which describes the application of action \( a \) from \( s \) to \( s' \), where \(s' = T(s, a)\).

% The value function, \( Q(s, a) \), quantifies the expected reward from executing action \( a \) at state \( s \), defined by:

% \[
% Q(s, a) = \mathbb{E}[R(s') | s' = T(s, a)]
% \]

% The reward function $R(s')$ quantifies the desirability of transitioning to a new state $s'$. This function evaluates the correctness and quality of the solution represented by $s'$, typically employing a model-specific scoring mechanism. The policy function $\pi(s)$ establishes a mapping from the state space to the action space. Of particular significance is the optimal policy $\pi^*(s)$, which, for any given state $s$, selects the action $a$ that maximizes the value function $Q(s,a)$. This formulation ensures the selection of actions that yield the highest expected utility.

% \[
% \pi^*(s) = \arg\max_{a \in A(s)} Q(s, a)
% \]

% This representation underscores the dynamic and iterative nature of decision-making in mathematical problem-solving, emphasizing continuous refinement and optimization of solutions through strategic action selection based on evaluated rewards.

% 感觉这里还需要有一段，来说明一下2.3， 2.4， 2.5之间的关联关系，以及如何来相互作用来解决preliminary提出的那个核心问题。这样就前后呼应，形成一个整体。


% Unlike MCTSr~\citep{zhang2024accessinggpt4levelmathematical} where a prompt-based scoring metric generated by LLMs is applied to reflect the correctness of answers, we want to use a pairwise scoring metric joint with insertion sort~(details in Algorithm~\ref{appendix:calc_reward} of Appendix A) to have a fair ranking of answers and avoid LLM hallucination~\citep{}.

% We use PRM800k~\citep{lightman2023let} to train our pairwise reward model or reuse reward model from FLAMe~\citep{vu2024foundational}. RewardBench~\citep{lambert2024rewardbench}

% DPRM encompasses DPO~\citep{rafailov2024direct}, 

% In mathematical tasks, the challenge of reward annotation is addressed through the implementation of process reward models and outcome reward models. By integrating these approaches, a comprehensive dataset incorporating samples from both process and outcome rewards was constructed to generate a substantial volume of mathematical preference dataset. Subsequently, a pairwise preference function $ f: A \times A \to \{\prec, =, \succ\} $, can be developed to judge the partial ordering relations among mathematical solutions.

% In practice, we employ a reward model $P$ parameterized by $\phi$ to predict the probability that a certain partial order relationship holds between two elements $a_1$ and $a_2$ as follows:
% $$
% P(a_1 \succ a_2 | \phi) = \frac{e^{\phi(a_1)}}{e^{\phi(a_1)} + e^{\phi(a_2)}}
% $$
% Inspired by advances in language interface fine-tuning (LIFT), we have transformed the task of modeling pairwise preference rewards into a question-answering task to ascertain the validity of partial-order relations.  Then pairwise preference reward model (PPRM) $\pi$ parameterized by $\phi$ in question-answering form can be formalized as follows:
% $$
% \pi(q,a_1,a_2 |\phi ) = 
% \begin{cases} 
% \text{yes} ,& \text{if } a_1 \succ a_2, \\
% \text{no} ,& \text{if }  a_1 \prec a_2
% \end{cases}
% $$

% The reward function for this question-answering task is formalized as follows:


% $$
% R(\hat{y}, y) = 
% \begin{cases} 
% 1 ,& \text{if } \hat{y} = y, \\
% 0 ,& \text{if } \hat{y} \neq y 
% \end{cases}
% $$
% The pairwise preference dataset $\mathcal{D}$ are converted into a dataset $\mathcal{D}^{'}$suitable for a question-answering framework, where we employ reinforcement learning with human feedback (RLHF) techniques to train the model, aiming to improve answer generation for the partial-order prediction question-answering task. Then, we employ the Direct Preference Optimization (DPO) method to find the optimal $\pi_\phi$ for following objective:

% $$
% \arg\max_{\phi} \mathbb{E}_{\pi}[R(\hat{y}, y)]
% $$

% To extrapolate a global advantage from locally derived binary partial orders, it is essential to synthesize these local rankings into a cohesive global ranking. This synthesis addresses the challenge of the global optimal ranking aggregation problem. Although the Kemeny-Young method, adhering to the Condorcet criterion, offers an optimal solution, its computational expense is significant. The method requires calculating the inconsistency of each ranking list, such as the number of inversions (inversion number) and Kendall's tau coefficient, processes that are computationally intensive with costs estimated at \(\mathbf{O}(n^3)\), often rendering it impractical. As an alternative, we propose a method predicated on the assumption of transitivity: a Borda count methodology enhanced by the Floyd-Warshall algorithm for transitive closure.

% Our dual-faceted approach integrates local win rates with global quantiles to compute the \( Q \)-value for each solution. Local win rates provide immediate, context-specific rewards indicative of short-term performance, while global quantiles, derived from an aggregated ranking, offer a comprehensive assessment of each solution's overall effectiveness. This integration of local assessments with a global overview establishes a robust metric for evaluating potential solutions.

% The computation of global quantiles is vital for navigating the complexities of optimal rank aggregation. Due to the substantial computational demands of the Kemeny-Young method, our approach leverages an assumption of transitivity among pairwise dominance relations, employing a Borda count algorithm enhanced by the Floyd-Warshall algorithm for transitive closure. This algorithm determines the transitive closure among solutions, thereby solidifying preference relationships. Rankings are then assigned based on these established dominance hierarchies. In instances where solutions have equivalent win counts, additional sampling of partial orders is conducted to refine their relative standings. The aggregation of these Borda count rankings enables the computation of quantiles, thus providing a scalable and computationally efficient method for global evaluation. This integration of methodologies enhances the coherence of our approach and ensures a robust framework for deriving comprehensive solution assessments.

% 数学解题任务的马尔科夫决策形式化

% - 数学解题任务可以被建模为一种搜索优化问题，从而应用蒙特卡洛树方法来进行优化
% 数学解题任务状态空间和动作空间的的形式化有三种思路，我们称之为工作于词元级别的(token-wise)、工作于步骤级别的（step-wise）、基于完整答案级别的（full-answer-wise） 
% - 工作于词元级别的可以视作一种启发式的解码策略，其复杂度不足以在任务中实际运用复杂的数学知识，但在低级任务的视角上提供了强大的灵活性
% - 工作于步骤级别的方法主要受COT范式的启发，将解题过程建模为多个步骤，其状态空间是已有的步骤序列，动作空间在已有的序列的基础上，续写扩展新的步骤，直到获得最终答案
% - 工作于完整答案级别的数学解题方法主要受到self-refine工作的启发，其状态空间是完整的答案，而动作空间是对一个既有答案的refine，由critic和rewrite两个步骤组成；

% xx等人的研究中，单步的self-refine和序列化的self-refine，对于数学任务表现出强大的潜力，但是序列化的的决策方式是naive的，缺少回溯、启发式的步骤选择和剪枝等对复杂搜索决策任务来说关键的特性；xx等人的工作中，蒙特卡洛树搜索与工作于步骤级别的方法的结合也展现了强大的性能；（xx等人建议，工作于完整答案级别的方法优于步骤级别方法，具有更好的数学知识运用和鲁棒性；分步骤的数据与全句级别的训练数据相比更加稀缺；）因此，我们尝试将蒙特卡洛树搜索方法与self-refine相结合，提出了MCTSr方法；
    

% - 为此，我们将数学解题任务定义为一种基于搜索的黑盒优化任务；
% - 其状态空间是一条完整的解题答案；动作空间是对旧答案的一次改写；
% - 对于一个数学问题，我们将一个答案作为一个状态，将所有可能的答案构成的空间作为搜索任务的状态空间；
% - 我们定义价值函数Q，对于一个状态（答案），给出一个标量反馈；
%     - 对于一个数学问题，存在一个最优状态，作为其最优解，其Q价值高于任意其他状态；
% - 我们定义动作空间；
%     - 一个旧答案和其经过改写函数后得到的新答案组成一个改写对；动作空间定义在所有可到达的改写对上；
%     - 动作空间基于改写对的概念，对于任意已有答案和改写函数推出的所有可到达改写对，构成由当前状态到新状态的可选动作；动作执行后，状态由原答案转移到新答案；
%     - 工作于完整答案级别的方法具有马尔可夫性质，改写动作只依赖于当前状态；
%     - 只考虑单步决策的情况下，最优动作的定义是，对于一个状态，存在一个可到达的改写对，对于任意其他改写对，其转移后的新状态的价值都是最高的；

% - 基于状态空间和动作空间的定义，策略函数是从状态空间到动作的映射；
%     - 对于当前状态，策略函数给出一个可选的改写对;
%     - 只考虑单步转移决策的情况下，最优策略的定义，是对于任意状态，都可以给出一个可到达改写对作为最优动作。



% - 回顾经典MCTS方法的架构
%     - 蒙特卡洛树搜索算法是一种强大的强化学习搜索方法，蒙卡树搜索属于马尔可夫决策的一种，其基本概念包含状态、动作和代价函数，蒙卡树通过采样的方式对这些函数进行蒙卡近似
%     - 蒙特卡洛树搜索算法有选择、展开、模拟/评估、反向传播四个步骤 
%         - 选择阶段的经典方法使用UCT方法，进行探索和利用的平衡
%         - 展开阶段...
%         - 评估或模拟
%         - 反向传播

% - 在以上定义的基础上，对于一个确定的数学问题，我们引入搜索树范式来规范求解其最优答案的过程；
%     - 其状态空间/搜索树上的节点是一条完整的解题答案；
%     - 动作空间/搜索树上的边是一对父节点的一次改写；
% - MCTSr方法基于经典蒙特卡洛树的架构，针对数学任务的特性进行了适应；
%     - 选择阶段，对于一棵改写树，选择阶段的目的是选择一个节点作为父节点以供展开，使得展开得到的新节点的Q价值更高；
%         - 我们使用UCT方法和Q价值函数进行节点的选择，以平衡探索和利用；
%         - 为了防止节点选择陷入局部最优，我们对可探索的节点的集合进行动态剪枝；
%             - 我们定义一个节点是完全探索的，当且仅当：
%                 - 子节点数量大于等于最大子节点数量；且
%                 - 存在子节点的Q价值大于此节点的Q价值
%     - 展开阶段，展开被选中的节点，得到新的节点，加入到搜索树中
%         - 我们定义一个改写函数，这个函数定义在状态空间上，是从当前状态向新状态的映射；
%             - 改写函数由一次self-critic和一次rewrite构成
%             - self-critic步骤中，模型对当前状态（答案）给出critique；
%             - rewrite步骤中，模型根据critique，对当前状态（答案）进行改写，得到一个新的答案；
%             - 理想条件下，这个映射应当能使的新状态的奖励函数价值优于旧状态；
%         - 为了简化问题，我们不对动作执行后的状态转移进行蒙特卡洛近似，仅使用贪婪策略，即我们假设改写动作执行后的状态转移是固定的；
%     - 评估阶段，我们使用PPRM对树中的节点进行偏序关系的采样；
%         - 得到的胜负矩阵计算Quantile，以评估节点的全局价值函数；
%         - 同时使用节点在树结构上的关系构成的局部胜负关系计算局部价值函数；
%         - 两者的组合构成节点最终的Q价值；
%         - 这种方法是对节点真实价值的一种蒙特卡洛近似。
%     - 反向传播阶段，我们从叶子节点出发，将子节点的价值Q向父节点以固定的折扣系数进行加和，作为对节点改进潜力的评估。 
% - 与基于步骤的方法使用得出最终答案作为叶子节点和终止边界不同，基于完整答案的方法没有严格的终止信号，因此我们使用总的rollouts，即搜索树中节点的数量来限制搜索树的规模和深度。
% - 在循环结束后，我们使用节点全局Q价值对节点进行排序。
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{image.png}
%     \caption{Enter Caption}
%     \label{fig:enter-label}
% \end{figure}

% \subsection{Derivation of Q-Value from Pairwise Preferences}

% Our study addresses the problem \( q \) with \( n \) potential solutions using a Partially Ordered Reward Model (PPRM). This model delineates pairwise preference relationships \( a_1 \succ a_2 \). We integrate Monte Carlo Tree Search (MCTS) with the Upper Confidence Bound (UCB) algorithm, incorporating reward functions at each node within the tree structure. This approach emphasizes the localized nature of reward calculations, constrained by the tree's structural parameters, and contrasts with the necessity for a global perspective across the entire reward spectrum. This juxtaposition between localized and global evaluations underpins our methodology, highlighting the intricate balance between immediate and strategic reward considerations in optimization processes.

% \cn{下面的部分还要重构}

% - PPRM 
%     - 数学解题答案间成对偏好关系的定义
%     - 结果奖励监督模型ORM和过程奖励监督模型PRM的定义都有局限性，我们受到DPO的启发，想直接建模两个答案之间的偏序关系
%     - PPRM数据集的构建
%     - sigmoid二元化奖励函数的定义，
%     - 利用lift将二元奖励函数建模转换为问答任务
%     - 使用RLHF和DPO损失函数来训练问答任务模型
% - 从局部二元奖励函数的偏序关系获取全局的排序
%     - Q函数由全局排序quantile和局部胜率的加权和构成
%     - 全局函数使用局部排序计算得来
%     - 传递闭包增强的波达计数算法
%         - 构造二元逻辑胜负矩阵M
%         - 定义胜负关系的传递性假设
%         - 使用图论中的floyd-warshall计算传递性闭包矩阵C
%         - 由图论中的出度概念，统计每个节点的胜负次数作为波达计数
%         - 对于胜负次数完全相同的节点，使用PPRM再计算一次胜负关系
%         - 得到最终的全局胜负排序，计算每个节点的quantile分数

% \textbf{Direct Preference Optimization (DPO):} To further improve the model's ranking ability, we introduce a Direct Preference Optimization (DPO) loss function. This loss function minimizes the discrepancy in partial ordering between the model \(\pi_\theta\) and a reference model \(\pi_{\text{ref}}\). The DPO loss is given by:

% \[
% L_{DPO}(\pi_\theta; \pi_{\text{ref}}) = -\mathbb{E}_{(x, y_u, y_l) \sim \mathcal{D}} \left[ \log \sigma \left( \beta \log \frac{\pi_\theta(y_u | x)}{\pi_{\text{ref}}(y_u | x)} - \beta \log \frac{\pi_\theta(y_l | x)}{\pi_{\text{ref}}(y_l | x)} \right) \right]
% \]

% By minimizing this loss function, the model can better simulate the relative ranking of solutions.


% Here, \( N(s) \) represents the number of times node \( s \) has been visited, \( N(s, a) \) denotes the times an action \( a \) has been taken from \( s \), and the parameter \( c \) represents a constant that regulates the magnitude of exploration within the algorithm. Following this, in the expansion phase, the chosen node \( s \) is expanded to generate all potential subsequent states \( s' \), which are then incorporated as new nodes into the tree \( \mathcal{T} \). The evaluation phase involves assessing these new nodes to estimate their Q values, often through simulations or heuristic methods, followed by the backpropagation phase where these Q values are propagated back from the leaf nodes to the root, updating the value estimates across the path.

==> figures/first_image.tex <==
\begin{tikzpicture}[node distance = 2cm, auto]
    % Part 1: Problem Explanation (left)
    \node [cloud] (problem) {复杂数学推理问题};
    \node [block, below of=problem, node distance=2cm] (complex) {无限动作空间};
    \node [block, below of=complex, node distance=2cm] (traditional) {传统方法受限};

    % Part 2: MCTSr Workflow (center)
    \node [block, right of=problem, node distance=6cm] (mctsr) {MCTSr 方法};
    \node [block, below of=mctsr, node distance=2cm] (node_select) {节点选择 (UCT)};
    \node [block, below of=node_select, node distance=2cm] (self_refine) {自我修正与状态改写};
    \node [block, below of=self_refine, node distance=2cm] (backprop) {回溯与更新};

    % Part 3: Results (right)
    \node [cloud, right of=mctsr, node distance=6cm] (result) {实验结果};
    \node [block, below of=result, node distance=2cm] (sota) {SOTA 表现};
    \node [block, below of=sota, node distance=2cm] (datasets) {GSM8K \& MATH 数据集};

    % Draw lines between nodes
    \path [line] (problem) -- (complex);
    \path [line] (complex) -- (traditional);

    \path [line] (mctsr) -- (node_select);
    \path [line] (node_select) -- (self_refine);
    \path [line] (self_refine) -- (backprop);

    \path [line] (result) -- (sota);
    \path [line] (sota) -- (datasets);

    % Draw connections between sections
    \path [line] (traditional) -- (mctsr);
    \path [line] (backprop) -- (result);

\end{tikzpicture}

==> note.tex <==


\subsection{备忘}
pass@k的原始论文
https://arxiv.org/pdf/2107.03374


MATH500是出自PRM800K的测试集，是MATH的更难的子集

\section{Todo}



\subsection{已完成}
\begin{itemize}
    \item \section{工程设定}
\end{itemize}
\subsection{1.偏好奖励模型}

\subsection{pairwise preference dataset}

    \begin{itemize}
        \item prm800k
    \end{itemize}
    https://github.com/openai/prm800k
    \begin{itemize}
        \item 合成脚本
    \end{itemize}
    https://github.com/AI4Chem/CriticMath
    
\subsection{pairwise reward model}
    
    \begin{itemize}
        \item FLAMe
    \end{itemize}
    https://arxiv.org/abs/2407.10817 

\subsection{2.mctsr 框架修改}
https://github.com/jianbo27/Refined-MathBlackBox
    reward function
    terminate function



\section{evaluation设定}
！！证明self-evaluation不可靠
采样n次答案，选出错误的m次，和gt一起让llm重排，来证明自重排不可靠

\subsection{3.benchmark dataset}
Olympiad，gsm， MATH

\subsection{一步回答：}
GPT-4O
GPT-4
Gemini pro
claude
deepseek-math
mumath
internlm-math

\subsection{self-refine方法:}
self-refine
naive mctsr
tree of thought
self-consistency


\subsection{基线模型}
llama3.1
gpt-4o mini


时间线和TOdo
2024.8.3
\begin{itemize}
    \item zhang
\end{itemize}
由prm800k合成pairwise preference dataset
\begin{itemize}
    \item wu
\end{itemize}
FLAMe
\begin{itemize}
    \item lei
\end{itemize}
！！证明self-evaluation不可靠
采样n次答案，选出错误的m次，和gt一起让llm重排，来证明自重排不可靠


==> tables/terminology.tex <==
\begin{table}[!htbp]
    \centering
    \caption{Notation Used}
    \label{tab:terminology}
    \begin{tabular}{|c|c|} \hline 
         \textbf{Variable} &  \textbf{Meaning}\\ \hline 
         $A$ & action space \\ \hline
         $\mathcal{D}$ &  pairwise preference dataset \\ \hline 
         $N(s)$ & the number of times node $s$ has been visited \\ \hline
         $P$ & reword model \\ \hline
         $Q$ & expected reward function \\ \hline
         $R$ & reward / loss function \\ \hline
         $S$ & state space \\ \hline
         $\mathcal{T}$ & state transition function \\ \hline
         $\textit{T}$ & maximum number of search steps \\ \hline
         $a_i$ &  edge i / action i \\ \hline
         $c$ & the extent of exploration \\ \hline
         $s_i$ &  node i / state i \\ \hline
         $t_i$ & search step i \\ \hline
         $\gamma$ & discount factor \\ \hline
         $\phi$ & parameters of reword model \\ \hline 
         $\pi$ & pairwise preference reward model \\ \hline
    \end{tabular}
\end{table}
